Towards Situation Awareness and Attention Guidance in a Multiplayer Environment using Augmented Reality and Carcassonne

Augmented reality (AR) games are a rich environment for researching and testing computational systems that provide subtle user guidance and training. In particular computer systems that aim to augment a user's situation awareness benefit from the range of sensors and computing power available in AR headsets. In this work-in-progress paper, we present a new environment for research into situation awareness and attention guidance (SAAG): an augmented reality version of the board game Carcassonne. We also present our initial work in producing a SAAG pipeline, including the creation of game state encodings, the development and training of a gameplay AI, and the design of situation modelling and gaze tracking systems.

==> sections/system.tex <==
\subsection{System Overview}
\label{sec:overview}

One major challenge in the production of these models is the lack of available gameplay data.
We considered a number of approaches for gathering this data for model training.
One option that was considered was to process available Carcassonne playthrough videos that can be found, for example, on Twitch.
However, we decided that the process would be too cumbersome and would not produce enough data.

Instead, we decided to build and train a gameplay AI to learn the game and produce gameplay data through self-play.
That data could eventually be augmented by human player data as people began to test the AR version of the game that we produce.
